Quantized Berry Phases for a Local Characterization of Spin Liquids in Frustrated Spin Systems

Recently by using quantized Berry phases, a prescription for a local characterization of gapped topological insulators is given. One requires the ground state is gapped and is invariant under some anti-unitary operation. A spin liquid which is realized as a unique ground state of the Heisenberg spin system with frustrations is a typical target system, since pairwise exchange couplings are always time-reversal invariants even with frustrations. As for a generic Heisenberg model with a finite excitation gap, we locally modify the Hamiltonian by a continuous SU(2) twist only at a specific link and define the Berry connection by the derivative. Then the Berry phase evaluated by the entire many-spin wavefunction is used to define the local topological order parameter at the link. We numerically apply this scheme for several spin liquids and show its physical validity.

==> mydef.tex <==
\newcommand{\nm}[3]{
\begin{xy}
0*=<#2mm,#3mm>[F]{\mb{ #1}}="box";
"box"%+U*!D\txt\small{$M$\\ \, }
,
"box"%+L*!R\txt\small{\, $N$\\ }
\end{xy}}
\newcommand{\nms}[5]{
\begin{xy}
0*=<#4mm,#5mm>[F]{\mb{ #1}}="box";
"box"+U*!D\txt\small{$#3$\\ \, }
,
"box"+L*!R\txt\small{\, $#2$\\ }
\end{xy}}
%
\newcommand{\nmmat}[5]{
\,
\begin{xy}0;<#5mm,#5mm>:
(0,0.5)*=<#5mm,#5mm>[F]{\mb{#1}}="box";
(-0.5,0)*=<#5mm,#5mm>[F]{\mb{#3}}="box";
(0.5,0)*=<#5mm,#5mm>[F]{\mb{#2}}="box";
(0,-0.5)*=<#5mm,#5mm>[F]{\mb{#4}}="box";
\end{xy}
}

\newcommand{\PCvec}[3]{
\begin{xy}0;<#3mm,#3mm>:
(0,1.0)*=(1,2)[F]{\mb{#1}}="box";
(-0.5,0)*=(1,2)[F]{\mb{#2}}="box";
\end{xy}
}
\newcommand{\rvec}[3]{
\begin{xy}
0*=<#1mm,#1mm>[F]{\mb{#2}}="box";
<#1mm,0mm>*=<#1mm,#1mm>[F]{\mb{#3}}="box";
\end{xy}
}
\newcommand{\ket}[1]{|{#1} \rangle }
%\newcommand{\seceq}{  (\thesection - \theequation)}
\newcommand{\mb}[1]{\mbox{\boldmath $#1$}}
\newcommand{\aeq}[0]{&=&}
%
\newcommand{\mchs}[2]
{
\left\{
\begin{array}{l}
#1    \\
#2
\end{array}
\right.
}
%
\newcommand{\mchss}[4]
{
\left\{
\begin{array}{cc}
#1 & #2   \\
#3 & #4
\end{array}
\right.
}
%
\newcommand{\dmat}[2]
{
\left(
\begin{array}{cc}
#1 &  \\
 & #2 
\end{array}
\right)
}
\newcommand{\mats}[4]
{\scriptstyle
\left(
\begin{array}{cc}
#1 & #2 \\
#3 & #4 
\end{array}
\right)
}
\newcommand{\smat}[4]
{
\begin{array}{cc}
#1 & #2 \\
#3 & #4 
\end{array}
}
\newcommand{\matthree}[9]
{
\left(
\begin{array}{ccc}
#1 & #2 & #3 \\
#4 & #5 & #6 \\
#7 & #8 & #9 
\end{array}
\right)
}
%
\newcommand{\matthrees}[9]
{\small
\left(
\begin{array}{ccc}
#1 & #2 & #3 \\
#4 & #5 & #6 \\
#7 & #8 & #9 
\end{array}
\right)
}
%
\newcommand{\wmvec}[2]
{
\begin{array}{c}
#1  \\
#2  
\end{array}
}
\newcommand{\mvecs}[2]
{\small
\left(
\begin{array}{c}
#1  \\
#2  
\end{array}
\right)
}
\newcommand{\mvec}[2]
{\small
\left(
\begin{array}{c}
#1  \\
#2  
\end{array}
\right)
}
%
\newcommand{\msvec}[2]
{
\begin{array}{c}
#1  \\
#2  
\end{array}
}
%
\newcommand{\mvecthree}[3]
{
\left(
\begin{array}{c}
#1  \\
#2  \\
#3  
\end{array}
\right)
}
%
\newcommand{\mvecfour}[4]
{
\left(
\begin{array}{c}
#1  \\
#2  \\
#3  \\
#4  
\end{array}
\right)
}
%
\newcommand{\mvecfive}[5]
{
\left(
\begin{array}{c}
#1  \\
#2  \\
#3  \\
#4  \\
#5  
\end{array}
\right)
}
%
\newcommand{\mvecsix}[6]
{
\left(
\begin{array}{c}
#1  \\
#2  \\
#3  \\
#4  \\
#5  \\
#6  
\end{array}
\right)
}
%
\newcommand{\minv}[1]{#1^{-1}}
\newcommand{\minfty}[0]{{-\infty}}
\newcommand{\cosec}[0]{{\rm \ cosec}}
\newcommand{\im}[0]{{\rm Im\ }}

\newcommand{\mvs}[0]{\vskip 0.5cm}

